Implementing Security Protocol Monitors

Cryptographic protocols are often specified by narrations, i.e., finite sequences of message exchanges that show the intended execution of the protocol. Another use of narrations is to describe attacks. We propose in this paper to compile, when possible, attack describing narrations into a set of tests that honest participants can perform to exclude these executions. These tests can be implemented in monitors to protect existing implementations from rogue behaviour.

==> eptcsdata.tex <==
\providecommand{\firstpage}{22}
\providecommand{\publicationstatus}{T. Kutsia (Ed.): Symbolic Computation \\
in Software Science (SCSS'21)
\\
EPTCS 342, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.342.3}{10.4204/EPTCS.342.3}}

